The Stationary Prophet Inequality Problem

We study a continuous and infinite time horizon counterpart to the classic prophet inequality, which we term the stationary prophet inequality problem. Here, copies of a good arrive and perish according to Poisson point processes. Buyers arrive similarly and make take-it-or-leave-it offers for unsold items. The objective is to maximize the (infinite) time average revenue of the seller. Our main results are pricing-based policies which (i) achieve a $1/2$-approximation of the optimal offline policy, which is best possible, and (ii) achieve a better than $(1-1/e)$-approximation of the optimal online policy. Result (i) improves upon bounds implied by recent work of Collina et al. (WINE'20), and is the first optimal prophet inequality for a stationary problem. Result (ii) improves upon a $1-1/e$ bound implied by recent work of Aouad and Sarita\c{c} (EC'20), and shows that this prevalent bound in online algorithms is not optimal for this problem.

==> conclusion.tex <==
\section{Conclusion and Open Questions}
\todo{Flesh out, if have time}
In this work, ...

Natural questions: improve the bounds we obtain. For competitive algorithms, 
our single-good algorithm is optimal, and so the only remaining question is to nail down the optimal dependence on $C$.
Lower bound has a vanishingly small probability of multiple items, so seems plausible that $C=1$ suffices to achieve the same bounds. 
For online algorithms, we obtain a $0.656$-competitive algorithm. We note that our LP cannot be used to obtain much tighter bounds, since there exist instances $\calI$
for which 
Finally, for the multi-good problem, 


==> mechanism-design.tex <==

%\begin{comment}
\section{Implications for mechanism design}
\label{sec:mechanism-design}

% Results for the classic prophet inequality, such as those of \cite{samuel-cahn1984,niazadeh2018prophet} to name just a few, have direct implications for mechanism design, and we find that this connection holds for the stationary prophet inequality problem as well.
As discussed in \Cref{sec:intro}, much of the work on the classic prophet inequality problem has focused on pricing-based algorithms, which are appealing not only for their simplicity and strong economic interpretation, but also for their implications in mechanism design.
We find that similar results hold for the single-good stationary prophet inequality problem.

\subsection{Approximate welfare maximization}

In particular, we can view the fixed-threshold policy from \Cref{alg:main} as a randomized posted-price mechanism which is in fact weakly dominant-strategy incentive compatible (DSIC) and individually rational, meaning that each buyer's dominant strategy is to truthfully bid his private value for the good and no buyer is worse off by participating in the marketplace.

\begin{restatable}{cla}{WDSIC}
\label{cla:WDSIC}
A randomized posted-price mechanism $(\bar v, \bar p)$ for the stationary prophet inequality problem is weakly DSIC and individually rational.
\end{restatable}

See \Cref{appendix:mechanism-design} for proof.

Under a randomized posted-price mechanism, every buyer sold an item is charged the same price $\bar v$ regardless of his bid $b$ or private value $v$.
The welfare generated by a sale is the sum  of the buyer's utility $v - \bar v$ and the seller's revenue $\bar v$, yielding a total welfare of $v$.
Therefore, the approximations from \Cref{thm:1/2-competitive-single-good-policy,thm:0.656-approximate-single-good-policy} hold when comparing the performance of \Cref{alg:main} implemented as a posted-price mechanism to the welfare-maximizing offline and online mechanisms.
% Furthermore, by the equivalence between expected revenue and expected virtual welfare (cite), this posted-price mechanism is also $\nicefrac{1}{2}$- and $0.656$-approximations of the WDSIC revenue-maximizing offline and online mechanisms, respectively.\footnote{Although the value distribution $\calD$ is not necessarily regular, maximizing the ironed virtual surplus generates at least as much expected revenue in expectation (cite).}

% Therefore, by \Cref{thm:1/2-competitive-single-good-policy,thm:0.656-approximate-single-good-policy}, \Cref{alg:main} implemented as a posted-price mechanism is a $\nicefrac{1}{2}$- and $0.656$-approximation of the welfare-maximizing offline and online mechanisms, respectively.

\subsection{Approximate revenue maximization}

Consider a mechanism $\calM$ for the single-good stationary prophet inequality problem.
Let $\pi_\calM (b, \mathbf{b}_{-})$ denote the probability that a buyer who bids $b$ for the good is sold an item under $\calM$ when all other buyers bid $\mathbf{b}_{-}$ and let $p_\calM (b, \mathbf{b}_{-})$ denote the expected price paid.
We define the utility of a buyer with private value $v$ who bids $b$ for the good under mechanism $\calM$ by
\[ u_\calM (v, b, \mathbf{b}_{-}) = v \cdot \pi_\calM (b, \mathbf{b}_{-}) - p_\calM (b, \mathbf{b}_{-}). \]
The welfare generated is simply the buyer's utility plus the seller's revenue, or
\[ u_\calM (v, b, \mathbf{b}_{-}) + p_\calM (b, \mathbf{b}_{-}) = v \cdot \pi_\calM (b, \mathbf{b}_{-}). \]
When the context is unambiguous, we omit the subscript $\calM$ and drop $\mathbf{b}_{-}$ for simplicity of notation.

An important thing to keep in mind throughout this discussion is that for the randomized posted-price mechanism $\calM$ from \Cref{alg:main}, neither $\pi_\calM$ nor $p_\calM$ is actually prescribed by the mechanism\textemdash both are properties of this mechanism.

\begin{comment}

\subsubsection{When $\calD$ is continuous}

Suppose the distribution $\calD$ of buyers' private values for the good is continuous on the interval $[v_\text{min}, v_\text{max}]$ with density $f$ and cumulative density $F(v) = \int_{v_\text{min}}^v f(z) dz$.

\begin{thm}[Myerson's lemma]
\label{thm:Myerson-lemma-continuous}
A mechanism $\calM$ for the single-good stationary prophet inequality problem is (weakly) DSIC if and only if
\begin{enumerate}
    \item (monotonicity) holding $\mathbf{b}_{-}$ constant, $\pi_\calM (\cdot, \mathbf{b}_{-})$ is non-decreasing, and
    \item (price identity) for all $b \in [v_\text{min}, v_\text{max}]$,
    \[ p_\calM (b, \mathbf{b}_{-}) = b \cdot \pi_\calM (b, \mathbf{b}_{-}) - \int_{v_\text{min}}^b \pi_\calM (z, \mathbf{b}_{-}) dz.\footnote{Assuming $\pi_\calM (b, \mathbf{b}_{-})$ is differentiable. By standard advanced calculus, the same formula holds more generally for an arbitrary monotone function $\pi_\calM (b, \mathbf{b}_{-})$, including piecewise constant functions, for a suitable interpretation of the derivative $\frac{\partial}{\partial b} \pi_\calM (b, \mathbf{b}_{-})$ and the corresponding integral.} \]
\end{enumerate}
\end{thm}

\begin{proof}
We first prove the forward direction.
Assume mechanism $\calM$ is DSIC, fix a buyer, and fix the bids $\mathbf{b}_{-}$ of all other buyers.
In this case, for any $b, b^\prime \in [v_\text{min}, v_\text{max}]$, we have
\[ u(b, b, \mathbf{b}_{-}) \geq u(b, b^\prime, \mathbf{b}_{-}) \Rightarrow b \cdot \pi(b, \mathbf{b}_{-}) - p(b, \mathbf{b}_{-}) \geq b \cdot \pi(b^\prime, \mathbf{b}_{-}) - p(b^\prime, \mathbf{b}_{-}) \]
and 
\[ u(b^\prime, b^\prime, \mathbf{b}_{-}) \geq u(b^\prime, b, \mathbf{b}_{-}) \Rightarrow b^\prime \cdot \pi(b^\prime, \mathbf{b}_{-}) - p(b^\prime, \mathbf{b}_{-}) \geq b^\prime \cdot \pi(b, \mathbf{b}_{-}) - p(b, \mathbf{b}_{-}), \]
where for convenience we drop the subscript $\calM$.
Combining these two inequalities yields
\begin{equation}
\label{eq:DSIC-sandwich-continuous}
    b \cdot \left( \pi(b^\prime, \mathbf{b}_{-}) - \pi(b, \mathbf{b}_{-}) \right) \leq p(b^\prime, \mathbf{b}_{-}) - p(b, \mathbf{b}_{-}) \leq b^\prime \cdot \left( \pi(b^\prime, \mathbf{b}_{-}) - \pi(b, \mathbf{b}_{-}) \right).
\end{equation}
Without loss of generality, suppose $b \leq b^\prime$.
Then
\[ b \cdot \left( \pi(b^\prime, \mathbf{b}_{-}) - \pi(b, \mathbf{b}_{-}) \right) \leq b^\prime \cdot \left( \pi(b^\prime, \mathbf{b}_{-}) - \pi(b, \mathbf{b}_{-}) \right) \]
from \Cref{eq:DSIC-sandwich-continuous} implies that $\pi(b^\prime, \mathbf{b}_{-}) - \pi(b, \mathbf{b}_{-}) \geq 0$, or equivalently that $\pi(b^\prime, \mathbf{b}_{-})$ is non-decreasing in $b$, thus proving the monotonicity property.
To prove the price identity, we divide \Cref{eq:DSIC-sandwich-continuous} by $b^\prime - b$ and take $b^\prime \downarrow b$, which yields
\[ \frac{\partial}{\partial b} p(b, \mathbf{b}_{-}) = b \cdot \frac{\partial}{\partial b} \pi(b, \mathbf{b}_{-}). \]
Integrating both sides, we have
\begin{align*}
    p(b, \mathbf{b}_{-}) - p(v_\text{min}, \mathbf{b}_{-}) &= \int_{v_\text{min}}^b z \cdot \frac{\partial}{\partial z} \pi(z, \mathbf{b}_{-}) dz \\
    &= z \cdot \pi(z, \mathbf{b}_{-}) \big|_{v_\text{min}}^b - \int_{v_\text{min}}^b \pi(z, \mathbf{b}_{-}) dz \\
    &= b \cdot \pi(b, \mathbf{b}_{-}) - v_\text{min} \cdot \pi(v_\text{min}, \mathbf{b}_{-}) - \int_{v_\text{min}}^b \pi(z, \mathbf{b}_{-}) dz.
\end{align*}
Recall that $u(v_\text{min}, v_\text{min}, \mathbf{b}_{-}) = v_\text{min} \cdot \pi(v_\text{min}, \mathbf{b}_{-}) - p(v_\text{min}, \mathbf{b}_{-})$, and therefore
\[ p(b, \mathbf{b}_{-}) = b \cdot \pi(b, \mathbf{b}_{-}) - \int_{v_\text{min}}^b \pi(z, \mathbf{b}_{-}) dz - u(v_\text{min}, v_\text{min}, \mathbf{b}_{-}). \]
Setting $u(v_\text{min}, v_\text{min}, \mathbf{b}_{-}) = 0$, or alternatively $p(v_\text{min}, \mathbf{b}_{-}) = v_\text{min} \cdot \pi(v_\text{min}, \mathbf{b}_{-})$, we see that the price identity does indeed hold.

We now prove the backwards direction.
Consider a mechanism $\calM$ and assume the induced sale probability $\pi_\calM$ is monotonic and the price identity holds for $p_\calM$.
% Assume the monotonicity property and price identity hold for the sale probability $\pi_\calM$ and expected price $p_\calM$ of a mechanism $\calM$.
Fix a buyer with private value $v$ and fix the bids $\mathbf{b}_{-}$ of all other buyers.
Consider any $\delta > 0$, and compare the buyer's utility of a truthful bid with the utility of any higher bid.
Dropping the subscript $\calM$, we have
\begin{align*}
    u(v, v, \mathbf{b}_{-}) - u(v, v + \delta, \mathbf{b}_{-}) &= v \cdot \pi(v, \mathbf{b}_{-}) - p(v, \mathbf{b}_{-}) - \left( v \cdot \pi(v + \delta, \mathbf{b}_{-}) - p(v + \delta, \mathbf{b}_{-}) \right) \\
    &= v \cdot \pi(v, \mathbf{b}_{-}) - v \cdot \pi(v, \mathbf{b}_{-}) + \int_{v_\text{min}}^v \pi(z, \mathbf{b}_{-}) dz - v \cdot \pi(v + \delta, \mathbf{b}_{-}) + (v + \delta) \cdot \pi(v + \delta, \mathbf{b}_{-}) - \int_{v_\text{min}}^{v+\delta} \pi(z, \mathbf{b}_{-}) dz \\
    &= \delta \cdot \pi(v + \delta, \mathbf{b}_{-}) - \int_v^{v+\delta} \pi(z, \mathbf{b}_{-}) dz \\
    &\geq \delta \cdot \pi(v + \delta, \mathbf{b}_{-}) - \delta \cdot \pi(v + \delta, \mathbf{b}_{-}) \\
    &= 0.
\end{align*}
This first two equalities follow from the definition of the buyer's utility and the price identity, while the inequality follows from the monotonicity of $\pi(\cdot, \mathbf{b}_{-})$.
Analogously, we have
\[ u(v, v, \mathbf{b}_{-}) - u(v, v - \delta, \mathbf{b}_{-}) \geq 0. \]
Therefore, $\delta = 0$ is optimal and mechanism $\calM$ is DSIC.
This completes the proof.
\end{proof}

\begin{lem}
\label{lem:revenue-equals-virtual-welfare}
For any (weakly) DSIC mechanism $\calM$ for the single-good stationary prophet inequality problem, any buyer with private value $v$, and any values $\mathbf{v}_{-}$ of all other buyers,
\begin{equation}
\label{eq:revenue-equals-virtual-welfare}
    \E_v \left[ p_\calM (v, \mathbf{v}_{-}) \right] = \E_v \left[ \phi (v) \cdot \pi_\calM (v, \mathbf{v}_{-}) \right],
\end{equation}
where $\phi(v) = v - \frac{1 - F(v)}{f(v)}$.
\end{lem}

\begin{proof}
Fix a buyer with value $v$ and the values $\mathbf{v}_{-}$ of all other buyers.
Since the mechanism is DSIC, by the price identity from \Cref{thm:Myerson-lemma-continuous} we have
\[ \E_v \left[ p(v, \mathbf{v}_{-}) \right] = \int_0^{v_\text{max}} p(b, \mathbf{v}_{-}) \cdot f(b) db = \int_0^{v_\text{max}} \left(b \cdot \pi(b, \mathbf{v}_{-}) - \int_{v_\text{min}}^b \pi(z, \mathbf{v}_{-}) dz \right) \cdot f(b) db. \]
Switching the order of integration in the second term on the right hand side, we have
\begin{align*}
    \E_v \left[ p(v, \mathbf{v}_{-}) \right] &= \int_{v_\text{min}}^{v_\text{max}} b \cdot \pi(b, \mathbf{v}_{-}) \cdot f(b) db - \int_{v_\text{min}}^{v_\text{max}} \pi(z, \mathbf{v}_{-}) \left( \int_z^{v_\text{max}} f(b) db \right) dz \\
    &= \int_{v_\text{min}}^{v_\text{max}} b \cdot \pi(b, \mathbf{v}_{-}) \cdot f(b) db - \int_{v_\text{min}}^{v_\text{max}} \pi(z, \mathbf{v}_{-}) \cdot \left(1 - F(z) \right) dz \\
    &= \int_{v_\text{min}}^{v_\text{max}} \left( b - \frac{1 - F(b)}{f(b)} \right) \cdot \pi(b, \mathbf{v}_{-}) \cdot f(b) db \\
    &= \int_{v_\text{min}}^{v_\text{max}} \phi(b, \mathbf{v}_{-}) \cdot \pi(b, \mathbf{v}_{-}) \cdot f(b) db \\
    &= \E_v \left[ \phi(v, \mathbf{v}_{-}) \cdot \pi(v, \mathbf{v}_{-}) \right]. \qedhere
\end{align*}
\end{proof}

This implies that the expected price paid by a buyer equals the expected virtual welfare generated.
Taking the expectation of \Cref{eq:revenue-equals-virtual-welfare} with respect to $\mathbf{v}_{-}$ and by the linearity of expectation, a direct consequence of \Cref{lem:revenue-equals-virtual-welfare} is that the expected revenue of a DSIC mechanism is equal to its expected virtual welfare.
We note that this is not necessarily the case for general (non-DSIC) mechanisms since the proof of the equivalence between expected revenue and expected virtual welfare relies entirely on the price identity from \Cref{thm:Myerson-lemma-continuous}.

We would like to take advantage of this equivalence to claim that \Cref{alg:main} can also be used to approximately maximize expected \emph{revenue}.
Consider the mechanism $\calM$ prescribed by \Cref{alg:main} in the virtual value setting (i.e., when we use the solution to the offline/online linear programs $\mathrm{LP}_\mathrm{off/on}$ where all instances of $v_j$ are replaced by $\phi(v_j)$).
Notice that by the same reasoning from the proof of \Cref{obs:alg-fixed-threshold}, if $\phi(v)$ is non-decreasing in $v$, then $\calM$ is a randomized posted-price mechanism and it follows from \Cref{cla:WDSIC} that $\calM$ is weakly DSIC.
As a result, by \Cref{lem:revenue-equals-virtual-welfare}, the expected revenue of this mechanism is equal to its expected virtual welfare.
However, what if $\phi(v)$ is not monotonically non-decreasing?
In this case, the sale probability $\pi_\calM$ may not necessarily be monotonic in the buyer's bid and $\calM$ is not guaranteed to be DSIC.

We can address this challenge by instead considering the \emph{ironed} virtual value function $\tilde \phi(v)$. Suppose $\phi(v)$ is decreasing on the interval $[a, b]$. Define the ironed virtual value function by
\[ \tilde \phi(v) =
    \begin{cases}
        \frac{\int_a^b \phi(z) f(z) dz}{F(b) - F(a)} & \text{if } v \in [a, b] \\
        \phi(v) & \text{otherwise}.
    \end{cases}
\]
That is, we simply ``iron'' the decreasing region of $\phi(v)$ by replacing all virtual values in that region by their average.
Clearly $\tilde \phi(v)$ is monotonic non-decreasing, and as a result the mechanism prescribed by \Cref{alg:main} in the ironed virtual value setting is DSIC.
As a result, the equivalence between the expected revenue and the expected ironed virtual welfare of this mechanism from \Cref{lem:revenue-equals-virtual-welfare} does indeed hold.
All that remains is to relate the expected ironed virtual welfare and the expected virtual welfare.
We do so via the following lemma.

\begin{lem}
\label{lem:revenue-leq-ironed-virtual-value}
For any (weakly) DSIC mechanism $\calM$ for the single-good stationary prophet inequality problem, any buyer, and any values $\mathbf{v}_{-}$ of other buyers,
\[ \E_v \left[ p_\calM (v, \mathbf{v}_{-}) \right] \leq \E_v \left[ \tilde \phi(v) \cdot \pi_\calM (v, \mathbf{v}_{-}) \right]. \]
\end{lem}

\begin{proof}
Fix a buyer with value $v$ and the values $\mathbf{v}_{-}$ of all other buyers.
By definition of $\tilde \phi(v)$, we have
\begin{align*}
    \E_v \left[ \tilde \phi(v) \cdot \pi(v, \mathbf{v}_{-}) \right] &= \int_{v_\text{min}}^{v_\text{max}} \tilde \phi(z) \cdot \pi(z, \mathbf{v}_{-}) \cdot f(z) dz \\
    &= \int_{v_\text{min}}^a \phi(z) \cdot \pi(z, \mathbf{v}_{-}) \cdot f(z) dz + \left( \frac{\int_a^b \phi(z) f(z) dz}{F(b) - F(a)} \right) \left( \int_a^b \pi(z, \mathbf{v}_{-}) \cdot f(z) dz \right) + \int_b^{v_\text{max}} \phi(z) \cdot \pi(z, \mathbf{v}_{-}) \cdot f(z) dz \\
    &= \dots +  \left( \int_a^b \phi(z) \cdot \frac{f(z)}{F(b) - F(a)} dz \right) \left( \int_a^b \pi(z, \mathbf{v}_{-}) \cdot \frac{f(z)}{F(b) - F(a)} dz \right) \cdot \left( F(b) - F(a) \right) + \dots.
\end{align*}
Recall that $\phi(\cdot)$ is decreasing on $[a, b]$ while $\pi(\cdot, \mathbf{v}_{-})$ is non-decreasing on this region due to the monotonicity property from \Cref{thm:Myerson-lemma-continuous}.
Therefore, we can lower bound the expression above via the Harris inequality:
\begin{align*}
    \E_v \left[ \tilde \phi(v) \cdot \pi(v, \mathbf{v}_{-}) \right] &\geq \dots +  \left( \int_a^b \phi(z) \cdot \pi(z, \mathbf{v}_{-}) \cdot \frac{f(z)}{F(b) - F(a)} dz \right) \cdot \left( F(b) - F(a) \right) + \dots \\
    &= \int_{v_\text{min}}^{v_\text{max}} \phi(z) \cdot \pi(z, \mathbf{v}_{-}) \cdot f(z) dz \\
    &= \E_v \left[ \phi(v) \cdot \pi(v, \mathbf{v}_{-}) \right] \\
    &= \E_v \left[ p(v, \mathbf{v}_{-}) \right],
\end{align*}
where the last equality follows from \Cref{lem:revenue-equals-virtual-welfare}.
\end{proof}

A direct corollary of \Cref{lem:revenue-leq-ironed-virtual-value} is that the expected revenue of any DSIC mechanism is at most the expected ironed virtual welfare under the same mechanism.

Now consider the  mechanism $\tilde \calM$ prescribed by \Cref{alg:main} in the ironed virtual value setting.
Since the ironed virtual value is monotonic, $\tilde \calM$ is a randomized posted-price mechanism which is DSIC by \Cref{cla:WDSIC}.
Therefore by \Cref{lem:revenue-equals-virtual-welfare}, the seller's expected revenue under $\tilde \calM$ is equal to the expected ironed virtual welfare, which by \Cref{thm:1/2-competitive-single-good-policy} is a $\nicefrac{1}{2}$-approximation of the ironed-virtual-welfare-maximizing offline mechanism $\tilde \calM^*$:
\[ \E_\mathbf{v} \left[ \tilde p_{\tilde \calM} (\mathbf{v}) \right] = \E_\mathbf{v} \left[ \tilde \phi(v) \cdot \tilde \pi_{\tilde \calM} (\mathbf{v}) \right] \geq \frac{1}{2} \cdot \E_\mathbf{v} \left[ \tilde \phi(v) \cdot \pi_{\tilde \calM^*} (\mathbf{v}) \right]. \]
The expected ironed virtual welfare under $\tilde \calM^*$ trivially upper bounds the same quantity under the mechanism $\calM_\text{DSIC}^*$ which maximizes the expected virtual welfare within the class of DSIC mechanisms:
\[ \E_\mathbf{v} \left[ \tilde \phi(v) \cdot \pi_{\tilde \calM^*} (\mathbf{v}) \right] \geq \E_\mathbf{v} \left[ \tilde \phi(v) \cdot \pi_{\calM_\text{DSIC}^*} (\mathbf{v}) \right]. \]
By \Cref{lem:revenue-leq-ironed-virtual-value}, the expected ironed virtual welfare under $\calM_\text{DSIC}^*$ is at least the expected revenue, so we have
\[ \E_\mathbf{v} \left[ \tilde \phi(v) \cdot \pi_{\calM_\text{DSIC}^*} (\mathbf{v}) \right] \geq \E_\mathbf{v} \left[ p_{\calM_\text{DSIC}^*} (\mathbf{v}) \right]. \]
Therefore, the mechanism from \Cref{alg:main} for the ironed virtual value setting is a $\nicefrac{1}{2}$-approximation of the revenue-maximizing DSIC offline mechanism.
By an analogous line of reasoning, it is also a $0.656$-approximation of the revenue-maximizing DSIC online mechanism.

\end{comment}

\subsubsection{When $\calD$ is discrete}

Suppose the distribution $\calD$ of buyers' private values for the good is discrete with support $\{v_1 < \cdots < v_m\}$.
Define $g(v_j) = \Pr_{v \sim \calD} \left[ v = v_j \right]$ and $G(v_j) = \sum_{\ell=1}^j g(v_\ell)$.
We present an analogue of Myerson's lemma from \cite{bergemann2007discrete} in the following theorem, with the main difference (in comprison to the continuous case) being that expected price is no longer unique.

\begin{thm}[\cite{bergemann2007discrete}]
\label{thm:Myerson-lemma-discrete}
A mechanism $\calM$ for the single-good stationary prophet inequality problem is DSIC if and only if
\begin{enumerate}
    \item (monotonicity) holding $\mathbf{v}_{-}$ constant, $\pi_\calM (\cdot, \mathbf{v}_{-})$ is monotone non-decreasing, and
    \item (price identity) for all $j = 1, \dots, m$,
    \[ p_\calM (v_j, \mathbf{v}_{-}) = v_j \cdot \pi_\calM (v_j, \mathbf{v}_{-}) - \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \tilde \pi_\calM(v_{\ell+1}, \mathbf{v}_{-}) \]
    for some $\tilde \pi_\calM(v_{j+1}, \mathbf{v}_{-}) \in [\pi_\calM(v_j, \mathbf{v}_{-}), \pi_\calM(v_{j+1}, \mathbf{v}_{-})]$.
\end{enumerate}
\end{thm}

\begin{proof}
We first prove the forward direction.
Fix a DSIC mechanism $\calM$ for the single-good stationary prophet inequality problem, fix a buyer with value $v_{j+1}$, and fix the values $\mathbf{v}_{-}$ of all other buyers.
Since $\calM$ is DSIC, the buyer's utility is
\[ u(v_{j+1}, v_{j+1}, \mathbf{v}_{-}) = v_{j+1} \cdot \pi(v_{j+1}, \mathbf{v}_{-}) - p(v_{j+1}, \mathbf{v}_{-}) \geq  u(v_{j+1}, v_j, \mathbf{v}_{-}) = v_{j+1} \cdot \pi(v_j, \mathbf{v}_{-}) - p(v_j, \mathbf{v}_{-}). \]
Similarly,
\[ u(v_j, v_j) = v_j \cdot \pi(v_j) - p(v_j) \geq  u(v_j, v_{j+1}) = v_j \cdot \pi(v_{j+1}) - p(v_{j+1}), \]
where for convenience we drop $\mathbf{v}_{-}$.
Subtracting the second from the first, we have
\begin{equation}
\label{eq:DSIC-sandwich-discrete}
    \left(v_{j+1} - v_j \right) \cdot \pi(v_j) \leq u(v_{j+1}, v_{j+1}) - u(v_j, v_j) \leq \left(v_{j+1} - v_j \right) \cdot \pi(v_{j+1}).
\end{equation}
Since $v_j < v_{j+1}$, \Cref{eq:DSIC-sandwich-discrete} implies $\pi(v_j) \leq \pi(v_{j+1})$, meaning the monotonicity property does indeed hold.

To prove the price identity, we sum \Cref{eq:DSIC-sandwich-discrete}, which yields
\[ \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \pi(v_\ell) \leq u(v_j, v_j) - u(v_1, v_1) \leq \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \pi(v_{\ell+1}), \]
or 
\begin{equation}
\label{eq:utility-formula-discrete}
    u(v_j, v_j) = \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \tilde \pi(v_{\ell+1}) + u(v_1, v_1)
\end{equation}
for some $\tilde \pi(v_{\ell+1}) \in \left[ \pi(v_\ell), \pi(v_{\ell+1}) \right]$ for each $\ell = 1, \dots, m-1$.
Since by definition $p(v_j) = v_j \cdot \pi(v_j) - u(v_j, v_j)$, rearranging \Cref{eq:utility-formula-discrete} we have
\[ p(v_j) = v_j \cdot \pi(v_j) - \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \tilde \pi(v_{\ell+1}) - u(v_1, v_1). \]
Setting $u(v_1, v_1) = 0$, or alternatively $p(v_1) = v_1 \cdot \pi(v_1)$, we see that the price identity does indeed hold.

\color{blue} We next prove the backwards direction. To do.
\end{proof}

We now relate the expected revenue of a DSIC mechanism to its expected virtual welfare.

\begin{lem}[\cite{bergemann2007discrete}]
\label{lem:revenue-leq-virtual-welfare-discrete}
For any DSIC mechanism $\calM$ for the single-good stationary prophet inequality, any buyer, and any values $\mathbf{v}_{-}$ of other buyers,
\begin{equation}
\label{eq:revenue-leq-virtual-welfare-discrete}
    \E_v \left[ p_\calM (v, \mathbf{v}_{-}) \right] \leq \E_v \left[ \omega (v) \cdot \pi_\calM (v, \mathbf{v}_{-}) \right],
\end{equation}
where $\omega(v_j) = v_j - (v_{j+1} - v_j) \cdot \frac{1 - G(v_j)}{g(v_j)}$ for $j = 1, \dots, m$ and $v_{m+1} = v_m$. If $\tilde \pi(v_{j+1}, \mathbf{v}_{-}) = \pi(v_j, \mathbf{v}_{-})$ for all $j = 1, \dots, m-1$, \Cref{eq:revenue-leq-virtual-welfare-discrete} holds with equality.
\end{lem}

\begin{proof}
Fix a DSIC mechanism $\calM$ for the single-good stationary prophet inequality problem, a buyer, and the values of all other buyers.
As $\calM$ is DSIC, by the price identity from \Cref{thm:Myerson-lemma-discrete} we have
\[ \E_v \left[ p (v) \right] = \sum_{j=1}^m p(v_j) \cdot g(v_j) = \sum_{j=1}^m \left( v_j \cdot \pi (v_j) - \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \tilde \pi(v_{\ell+1}) \right) \cdot g(v_j). \]
Switching the order of summation in the second term on the right hand side, we have
\begin{align*}
    \E_v \left[ p (v) \right] &= \sum_{j=1}^m v_j \cdot \pi(v_j) \cdot g(v_j) - \sum_{j=1}^{m-1} \left(v_{j+1} - v_j \right) \cdot \tilde \pi(v_{j+1}) \cdot \left( 1 - G(v_j) \right) \\
&= \sum_{j=1}^m \left( v_j - \left(v_{j+1} - v_j \right) \cdot \frac{\tilde \pi(v_{j+1})}{\pi(v_j)} \cdot \frac{1 - G(v_j)}{g(v_j)} \right) \cdot \pi (v_j) \cdot g(v_j) \\
    &\leq \sum_{j=1}^m \left( v_j - \left(v_{j+1} - v_j \right) \cdot \frac{1 - G(v_j)}{g(v_j)} \right) \cdot \pi (v_j) \cdot g(v_j) \\
    &= \sum_{j=1}^m \omega(v_j) \cdot \pi (v_j) \cdot g(v_j) \\
    &= \E_v \left[ \omega(v) \cdot \pi (v) \right],
\end{align*}
where the inequality follows from the fact that $\tilde \pi(v_{j+1}) \geq \pi(v_j)$ for all $j = 1, \dots, m-1$ and for convenience we define $v_{m+1} = v_m$.
\end{proof}

Taking the expectation of \Cref{eq:revenue-leq-virtual-welfare-discrete} with respect to $\mathbf{v}_{-}$ and by the linearity of expectation, a direct consequence of \Cref{lem:revenue-leq-virtual-welfare-discrete} is that the expected revenue of any DSIC mechanism is at most its expected virtual welfare.

Unfortunately, it is not necessarily the case that \Cref{eq:revenue-leq-virtual-welfare-discrete} holds with equality for the randomized posted-price mechanism $\calM$ of \Cref{alg:main}.
Suppose under $\calM$, the seller is never willing to sell to buyers with value $v_1, \dots, v_{j^*-1}$, is willing to sell to buyers with value $v_{j^*}$ with some probability in $(0, 1)$, and always willing to sell to buyers with value $v_{j^*+1}, \dots, v_m$.
In this case, for any values of the other buyers,
\[ 0 = \pi_\calM (v_1) = \dots = \pi_\calM(v_{j^*-1}) < \pi_\calM (v_{j^*}) < \pi_\calM (v_{j^*+1}) = \dots = \pi_\calM(v_m). \]
By \Cref{cla:WDSIC}, $\calM$ is DSIC and therefore the price identity from \Cref{thm:Myerson-lemma-discrete} holds:
\[ p_\calM (v_j) = v_j \cdot \pi_\calM (v_j) - \sum_{\ell=1}^{j-1} \left(v_{\ell+1} - v_\ell \right) \cdot \tilde \pi_\calM (v_{\ell+1}). \]
Now in order to demonstrate that the left hand side of \Cref{eq:revenue-leq-virtual-welfare-discrete} may be strictly less than the right hand side, we show that $\tilde \pi_\calM (v_{j^*+1}, \mathbf{v}_{-}) > \pi_\calM (v_{j^*}, \mathbf{v}_{-})$.
Since $\pi_\calM (v_j) = \pi_\calM (v_{j+1})$ for $j = 1, \dots, j^*-2, j^*+1, \dots, m-1$, clearly $\tilde \pi_\calM (v_{j+1}) = \pi_\calM (v_j)$ for $j = 1, \cdots, j^* - 2, j^*+1, \dots, m-1$.
Furthermore, we know the expected price paid by a buyer with value $v_{j^*}$ under $\calM$ is $v_{j^*} \cdot \pi_\calM (v_{j^*})$, and combining this with the price identity yields
\[ v_{j^*} \cdot \pi_\calM (v_{j^*}) =  v_{j^*} \cdot \pi_\calM (v_j) - \sum_{\ell=1}^{j^*-1} \left(v_{\ell+1} - v_\ell \right) \cdot \tilde \pi_\calM(v_{\ell+1}), \]
or
\[ \left(v_{j^*} - v_{j^*-1} \right) \cdot \tilde \pi_\calM(v_{j^*}) = 0. \]
Since $v_{j^*-1} < v_{j^*}$, this implies $\tilde \pi_\calM(v_{j^*}) = 0$ and therefore $\tilde \pi_\calM(v_{j^*}) = \pi_\calM(v_{j^*-1}).$ This same analysis for a buyer with value $v_{j^*+1}$ yields
\[ v_{j^*} \cdot \pi_\calM (v_{j^*+1}) = v_{j^*+1} \cdot \pi_\calM (v_{j^*+1}) -  \left(v_{j^*+1} - v_{j^*} \right) \cdot \tilde \pi_\calM(v_{j^*+1}), \]
from which it follows that $\tilde \pi_\calM(v_{j^*+1}) = \pi_\calM(v_{j^*+1}) > \pi_\calM(v_{j^*})$.

\paragraph{An example where the inequality from \Cref{lem:revenue-leq-virtual-welfare-discrete} is strict}
To make this more concrete, consider the following simple instance.
Suppose we have two buyer types with values $v_1 = 1, v_2 = 2$ and they have equal arrival rates (i.e., the probability that a buyer who arrives to the marketplace is of type 1 is $1/2$, and the same for type 2).
The virtual values for these buyers are $\omega(v_1) = 1 - (2 - 1) * \frac{1 - 1/2}{1/2} = 0$ and $\omega(v_2) = 2$.
Suppose we have a mechanism under which the seller is always willing to sell to buyers of type $2$ and willing to sell to buyers of type $1$ with some probability $p \in (0, 1)$.
The expected revenue of this mechanism (from a single buyer) is
\[ \frac{1}{2} \cdot (1 \cdot p + 1) \cdot \bbP[A \geq 1], \]
while the expected virtual weflare is
\[ \frac{1}{2} \cdot (0 \cdot p + 2) \cdot \bbP[A \geq 1] = \bbP[A \geq 1]. \]
Clearly, $\frac{1}{2} \cdot (1 \cdot p + 1) < 1$ for any $p \in (0, 1)$, and therefore the expected revenue of this mechanism is strictly less than the expected virtual welfare.
On the other hand, it is easy to see that if $p = 0$ (i.e., the seller posted price $2$) or $p = 1$ (the seller posted price $< 1$), then the expected revenue and expected virtual welfare are in fact equal.

As a result, it is not clear how to relate the expected revenue of a randomized posted-price algorithm to its expected virtual welfare when the buyers' value distribution is discrete.
One possible path forward, however, is to round the randomized posted-price algorithm $\calM$ from \Cref{alg:main} to a deterministic posted-price $\calM^\prime$.
We show first in \Cref{cla:randomized-rounded-to-deterministic} that we lose at most a $\nicefrac{1}{2}$ factor in doing so, and then in \Cref{lem:revenue-equals-virtual-welfare-discrete-deterministic} that \Cref{eq:revenue-leq-virtual-welfare-discrete} holds with equality for deterministic posted-price mechanisms.

\begin{restatable}{cla}{RandomizedRoundedToDeterministic}
\label{cla:randomized-rounded-to-deterministic}
For any randomized posted-price mechanism for the single-good stationary prophet inequality problem, there exists a deterministic posted-price mechanism with at least half the expected average welfare.
\end{restatable}

See \Cref{appendix:mechanism-design} for proof.

\begin{lem}
\label{lem:revenue-equals-virtual-welfare-discrete-deterministic}
For any deterministic posted-price mechanism $\calM$ for the single-good stationary prophet inequality problem,
\[ \E_v \left[ p_\calM (v, \mathbf{v}_{-}) \right] = \E_v \left[ \omega (v) \cdot \pi_\calM (v, \mathbf{v}_{-}) \right]. \]
\end{lem}

\begin{proof}
Fix a deterministic posted-price mechanism $\calM$ for the single-good stationary prophet inequality problem under which the seller is never willing to sell to buyers with value $v_1, \dots, v_{j^*-1}$ and always willing to sell to buyers with value $v_{j^*}, \dots, v_m$ for some $1 \leq j^* \leq m$
In this case,
\[ \pi_\calM (v_1) = \cdots = \pi_\calM (v_{j^*-1}) < \pi_\calM (v_{j^*}) = \cdots = \pi_\calM (v_m). \]
It follows from \Cref{cla:WDSIC} that $\calM$ is DSIC, and as a result, by \Cref{lem:revenue-leq-virtual-welfare-discrete} it suffices to show that $\tilde \pi_\calM (v_{j+1}) = \pi_\calM (v_j)$ for all $j = 1, \dots, m-1$.
Clearly this is true for $j = 1, \cdots, j^*-2, j^*, \cdots, m-1$, so all that remains is to show that $\tilde \pi_\calM (v_{j^*}) = \pi_\calM (v_{j*-1})$.
The expected price paid by a buyer with value $v_j^*$ under $\calM$ is $v_{j^*} \cdot \pi_\calM (v_{j^*})$, and combining this with the price identity from \Cref{thm:Myerson-lemma-discrete} yields
\[ v_{j^*} \cdot \pi_\calM (v_{j^*}) = v_{j^*} \cdot \pi_\calM (v_{j^*}) - \sum_{\ell=1}^{j^*-1} \left( v_{\ell+1} - v_\ell \right) \cdot \tilde \pi_\calM (v_{\ell+1}). \]
Since $\tilde \pi_\calM (v_{\ell+1}) = 0$ for $\ell = 1, \dots, j^*-2$, this simplifies to
\[ \left( v_{j^*} - v_{j^*-1} \right) \cdot \tilde \pi_\calM (v_{j^*}) = 0, \]
from which it follows that $\tilde \pi_\calM (v_{j^*}) = 0$ since $v_{j^*} - v_{j^*-1} > 0$.
As $ \pi_\calM (v_{j^*-1}) = 0$, we do indeed have $\tilde \pi_\calM (v_{j^*}) = \pi_\calM (v_{j^*-1})$, which completes the proof.
\end{proof}

\subsubsection{Ironing virtual values}

If the virtual values $\{\omega_1, \dots, \omega_m\}$, where for convenience we denote $\omega_j = \omega(v_j)$, are not monotone non-decreasing, then the mechanism $\calM$ prescribed by \Cref{alg:main} for the virtual value setting (i.e., using the solution to $\mathrm{LP}_\mathrm{off/on}$ where all instances of $v_j$ are replaced by $\omega_j$) is not guaranteed to be DSIC.
As a result, there is no clear way to bound the expected revenue under $\calM$ in terms of the expected virtual welfare as in \Cref{lem:revenue-leq-virtual-welfare-discrete}.
We can address this challenge by instead considering the \emph{ironed} virtual values $\tilde \omega_j$, as proposed in \cite{elkind2007discrete}.
We compute these ironed virtual values by first constructing a piecewise linear function consisting of $m$ segments whose slopes are $\omega_1, \dots, \omega_m$.
If the sequence of virtual values is not non-decreasing, this piecewise function is not convex, in which case we compute its lower envelope (which is convex by definition) and we set $\tilde \omega_j$ to be the slope of the segment of the lower envelope which corresponds to $\omega_j$.
More formally, denote $g_j = g(v_j)$ and $G_j = G(v_j)$ and let $H_j = \sum_{\ell=1}^j \omega(v_\ell) \cdot g(v_\ell)$.
Set $G_0 = H_0 = 0$ and let $L(\cdot) : [0,1] \rightarrow \R$ be the lower envelope of the set $\{(G_0, H_0), (G_1, H_1), \dots, (G_m, H_m) \}$.
Finally set $L_j = L(G_j)$, noting that $L_0 = H_0 = 0$ and $L_m = H_m$, and define $\tilde \omega_j = \left( L_j - L_{j-1} \right) / \left( G_j - G_{j-1} \right) = \left( L_j - L_{j-1} \right) / g_j$.

\begin{cla}[\cite{elkind2007discrete}]
\label{cla:ironed-virtual-values-monotone-discrete}
The sequence $\{ \tilde \omega_1, \dots, \tilde \omega_m\}$ is non-decreasing.
\end{cla}

\begin{proof}
Observe that by definition, $\tilde \omega_j$ is the slope of the lower envelope $L(\cdot)$ between $G_{j-1}$ and $G_j$, and since $L(\cdot)$ is convex, $\tilde \omega_j \leq \tilde \omega_{j+1}$.
\end{proof}

\Cref{cla:ironed-virtual-values-monotone-discrete} implies the mechanism $\calM$ from \Cref{alg:main} for the ironed virtual value setting is indeed DSIC, in which case \Cref{lem:revenue-leq-virtual-welfare-discrete} does apply. All that remains is to relate the expected ironed virtual welfare and the expected virtual welfare, which we do via the following lemma.

\begin{lem}[\cite{elkind2007discrete}]
\label{lem:revenue-leq-ironed-virtual-value}
For any DSIC mechanism $\calM$ for the single-good stationary prophet inequality problem, any buyer, and any values $\mathbf{v}_{-}$ of all other buyers,
\[ \E_v \left[ \tilde \omega(v) \cdot \pi_\calM (v, \mathbf{v}_{-}) \right] \geq \E_v \left[ \omega(v) \cdot \pi_\calM (v, \mathbf{v}_{-}) \right]. \]
\end{lem}

\begin{proof}
Fix a DSIC mechanism $\calM$, a buyer, and the values of all other buyers.
We have
\begin{align*}
    \E_v \left[ \tilde \omega(v) \cdot \pi_\calM (v) \right] &= \sum_{j=1}^m \tilde \omega_j \cdot \pi_\calM (v_j) \cdot g_j \\
    &= \sum_{j=1}^m \left(L_j - L_{j-1} \right) \cdot \pi_\calM (v_j) \\
    &= -\sum_{j=1}^m L_j \cdot \left(\pi_\calM (v_{j+1} - \pi_\calM (v_j) \right) - L_0 \cdot \pi_\calM (v_1) + L_m \cdot \pi_\calM (v_m).
\end{align*}
Recall that as the lower envelope, by definition $L_j \leq H_j$ for all $j = 1, \dots, m$, and also $L_0 = H_0$ and $L_m = H_m$.
Therefore,
\begin{align*}
    \E_v \left[ \tilde \omega(v) \cdot \pi_\calM (v) \right] &\geq -\sum_{j=1}^m H_j \cdot \left(\pi_\calM (v_{j+1} - \pi_\calM (v_j) \right) - H_0 \cdot \pi_\calM (v_1) + H_m \cdot \pi_\calM (v_m) \\
    &= \sum_{j=1}^m \left(H_j - H_{j-1} \right) \cdot \pi_\calM (v_j) \\
    &= \sum_{j=1}^m \left( \frac{H_j - H_{j-1}}{g_j} \right) \cdot \pi_\calM (v_j) \cdot g_j \\
    &= \sum_{j=1}^m \omega_j \cdot \pi_\calM (v_j) \cdot g_j \\
    &= \E_v \left[ \omega(v) \cdot \pi_\calM (v) \right]. \qedhere
\end{align*}
\end{proof}

\begin{lem}
There exists a DSIC mechanism for the single-good stationary prophet inequality problem whose expected revenue is a $\nicefrac{1}{4}$- and $0.328$-approximation of the revenue-maximizing offline and online DSIC mechanisms.
\end{lem}

\begin{proof}
Fix an instance $\calI$ of the single-good stationary prophet inequality problem and consider \Cref{alg:main} using the solution to $\mathrm{LP}_\mathrm{off}$ where all occurences of $v_j$ are replaced by their ironed virtual values $\tilde \omega(v_j)$.
By \Cref{cla:ironed-virtual-values-monotone-discrete}, the sequence $\{\tilde \omega_1, \dots, \tilde \omega_m\}$ is monotone non-decreasing and therefore the mechanism $\calM$ prescribed by \Cref{alg:main} in this setting is a (randomized) posted-price mechanism which is weakly DSIC by \Cref{cla:WDSIC}.
We have
\[ \E_\mathbf{v} \left[ \tilde \omega(\mathbf{v}) \cdot \pi_\calM (\mathbf{v}) \right] \geq \frac{1}{2} \cdot \max_{\calM \text{ offline}} \E_\mathbf{v} \left[ \tilde \omega(\mathbf{v}) \cdot \pi_\calM (\mathbf{v}) \right] \geq \frac{1}{2} \cdot \max_{\calM \text{ offline DSIC}} \ \E_\mathbf{v} \left[ \omega(\mathbf{v}) \cdot \pi_\calM (\mathbf{v}) \right] \geq \frac{1}{2} \cdot \max_{\calM \text{ offline DSIC}} \ \E_\mathbf{v} \left[ p_\calM (\mathbf{v}) \right], \]
where the first inequality is due to \Cref{thm:1/2-competitive-single-good-policy}, the second inequality trivially holds, and the third inequality follows from \Cref{lem:revenue-leq-virtual-welfare-discrete}.
Furthermore, by \Cref{cla:randomized-rounded-to-deterministic} we can round $\calM$ to a deterministic posted price policy $\calM^\prime$ with at least half the expected ironed virtual welfare:
\[ \E_\mathbf{v} \left[ \tilde \omega(\mathbf{v}) \cdot \pi_{\calM^\prime} (\mathbf{v}) \right] \geq \nicefrac{1}{2} \cdot \E_\mathbf{v} \left[ \tilde \omega(\mathbf{v}) \cdot \pi_\calM (\mathbf{v}) \right]. \]
By \Cref{lem:revenue-equals-virtual-welfare-discrete-deterministic}, the expected revenue under $\calM^\prime$ is equal to the expected ironed virtual value, and so we have
\[ \E_\mathbf{v} \left[ \tilde p_{\calM^\prime} (\mathbf{v}) \right] = \E_\mathbf{v} \left[ \tilde \omega(\mathbf{v}) \cdot \pi_{\calM^\prime} (\mathbf{v}) \right]. \]
Combining these yields
\[ \E_\mathbf{v} \left[ \tilde p_{\calM^\prime}(\mathbf{v}) \right] \geq \nicefrac{1}{4} \cdot \max_{\calM \text{ offline DSIC}} \ \E_\mathbf{v} \left[ p_\calM (\mathbf{v}) \right]. \]

The proof comparing to the revenue-maximizing online DSIC mechanism is almost identical and is therefore omitted here.
\end{proof}

\subsubsection{Related works}
\begin{itemize}
    \item \cite{chawla2010multi}: Assume continuous distributions \& appeal to virtual values and ironing
    \item \cite{chawla2008algorithmic}: Top of page 4 - assume continuous distributions, proof of main theorem relies on expected revenue = expected virtual welfare (see Lemma 9, which is needed for proof of Theorem 14)
\end{itemize}

==> preamble.tex <==
\newenvironment{wrapper}[1]
{
	\smallskip
	\begin{center}
		\begin{minipage}{\linewidth}
			\begin{mdframed}[hidealllines=true, backgroundcolor=gray!20, leftmargin=0cm,innerleftmargin=0.375cm,innerrightmargin=0.375cm,innertopmargin=0.375cm,innerbottommargin=0.375cm,roundcorner=10pt]
				#1}
			{\end{mdframed}
		\end{minipage}
	\end{center}
	\smallskip
}
